New Frontiers in IoT: Networking, Systems, Reliability, and Security Challenges

The field of IoT has blossomed and is positively influencing many application domains. In this paper, we bring out the unique challenges this field poses to research in computer systems and networking. The unique challenges arise from the unique characteristics of IoT systems such as the diversity of application domains where they are used and the increasingly demanding protocols they are being called upon to run (such as, video and LIDAR processing) on constrained resources (on-node and network). We show how these open challenges can benefit from foundations laid in other areas, such as, 5G cellular protocols, ML model reduction, and device-edge-cloud offloading. We then discuss the unique challenges for reliability, security, and privacy posed by IoT systems due to their salient characteristics which include heterogeneity of devices and protocols, dependence on the physical environment, and the close coupling with humans. We again show how the open research challenges benefit from reliability, security, and privacy advancements in other areas. We conclude by providing a vision for a desirable end state for IoT systems.

==> sec_IoT_testbeds.tex <==
\section{IoT testbeds}

% A reference
“BenchIoT: A benchmark for the things in the Internet of Things,” N Almakhdhub, A Clements, M Payer, S Bagchi. 49th IEEE/IFIP International Symposium on Dependable Systems and Networks (DSN).



\subsection{Desired characteristics}
We need to create usable testbeds and data sets that can be used for replicable advances in the field and also be used for competitions for IoT systems. This is a commonly expressed need in many domains and have led to substantive advancements and benefits in many such domains. The need for this in IoT has become critical.

We can take inspiration from the networking area that has created usable testbeds through NSF's US Ignite and PAWR programs.

\subsection{Current state}

\subsection{Desired end goal}

% Industry and Academia
Industry is leading the development of applications, and can help academia understand business models, but participants felt that academia had a role to play in developing application areas (e.g., sustainability related) and IoT technologies (e.g., privacy) that may not yet, or ever, have a compelling business model, but may have significant societal benefit. Industry can also contribute benchmarks and data sets, but academia will need to design testbeds that foster open standards and shared experimentation with an emphasis on reproducibility. On the education front, participants discussed a range of topics from whether to offer specialized degrees in IoT, to the need for ethics and security and privacy education in IoT. They also noted the lack of textbooks for IoT.

% Do we have benchmarks or problem models?

% What are successful examples of IoT testbeds? What are desirable characteristics of a (future) IoT testbed?

% What kinds of shared experimental infrastructure (reusable software, datasets) do we need?

==> sec_challenge_ML.tex <==
\section{Challenges in applying ML to IoT}

\subsection{Unique problems}
Machine learning techniques can be particularly useful in IoT systems because of two fundamental reasons,
\begin{enumerate}
    \item the large volume of data generated by sensors which will need automated processing to deduce actionable information from them; 
    \item the large number of heterogeneous IoT devices which will need automated learning of their behaviors and consequent automated management.
\end{enumerate}   

IoT will also likely push the boundaries of federated learning motivated by the fact that each individual device may be too resource constrained and by privacy requirements in IoT settings. In data-rich contexts, novel machine intelligence algorithms, such as deep neural network based inference, can be used as a general intelligence support engine. Neural networks offer a great portable representation, much like a language virtual machine (e.g., Java and Python), that makes it possible to distribute inference algorithms across edge and cloud machines, and control the amount of communication among them. 
Services might (i) generate deep neural network models (from client-supplied training data), (ii) help with (automatic) labeling of data sets, and (iii) perform model reduction (if needed for caching on the edge device). Generated models might be executed as appropriate on the server or client. This vision poses several challenges.

\subsection{Resource Economy}

\subsubsection{Model Reduction for IoT Devices}
Modern machine intelligence algorithms are heavy-weight. To run on a low-end IoT device, solutions have been developed in recent literature that significantly reduce the computational and memory needs of machine inference. Recent work shows that model reductions of orders of magnitude are possible. For example, a device can cache a reduced model that identifies a number of most frequent commands, leaving the more general (but rarely encountered) identification tasks to the cloud. Models can also be customized to the specific hardware. For example, rather than minimizing computational cost, a model that fully utilizes an available GPU will give a better quality/consumption trade-off.

\subsubsection{Data Compression and Inference Offloading} 
Communication between the resource-constrained IoT end-device and an edge-processing server needs to be compressed. The degree of compression may depend on the bandwidth available. Adaptive compression techniques were proposed to address the problem. Auto-encoder-like solutions allow asymmetric encoding/decoding where the IoT-device-side encoder (that compresses the data onto a lower-dimensional manifold) is lightweight, whereas the decoder (running on an edge-server) is more involved. Order-of-magnitude reduction in communication was shown.

\subsubsection{Efficient Server-side Scheduling}
Recent studies on deep learning have shown that improvements in result accuracy diminish with increased depth of the neural network. Hence, efficiency considerations suggest that once a desired quality is achieved, the service should refrain from executing additional layers. A scheduler may determine how many stages to execute of each pipeline to avoid diminishing returns. 

\subsection{Automatic Labeling}
Training machine learning algorithms requires a labeling effort. Since labels are hard to come by, a key challenge is to reduce the need for labeled data. Semi-supervised learning becomes highly desirable. A recently proposed approach uses Generative Adversarial Networks (GAN) to generate realistic fakes that complement labeled data. This GAN has three elements, one proposes labels for unlabeled samples, one fakes data to match desired labels, whereas the last tries to distinguish the resulting labeled samples from the original labeled ones. As the game proceeds, all three entities learn from each other ultimately producing labeled data samples that are hard to falsify. Empirical results show that these eventual artificially produced samples (including originally unlabeled data) help improve accuracy of learning applications almost as much as the ground-truth labels themselves.

\subsection{Rethinking Learning Foundations}
\subsubsection{Learning in the Frequency Domain}
IoT devices and sensors often measure physical phenomena that obey some laws of nature. Unlike other data domains (such as handwriting recognition), the physical nature of the measured phenomenon endows it with distinguishable signatures in the frequency domain. Yet, modern machine learning solutions are predominantly design for the time domain. For example, convolutional neural networks are inspired by finding spatial patterns in time-series data. If the data were in the frequency domain, the convolution operation would reduce to a multiplication operation. Recent work has shown that neural network inference quality in IoT contexts can be significantly improved if the operators performed by the network were redesigned for the frequency domain. 

\subsubsection{Deconvolution and Unfolding}
An interesting artifact of learning in the frequency domain is the feasibility of implementing novel operations such as frequency unfolding to recover original signals from ones that suffered a high degree of aliasing due to sampling at significantly reduced frequencies. These solutions, for example, enable the reconstruction of sounds (8-16KHz) from data captured by accelerometers (400Hz). 

\subsection{Data Prioritization}
A commonly overlooked challenge in machine inference contexts is one of data prioritization. When a human driver observes a scene, they instinctively prioritize regions of higher criticality in the scene (such as a child on the side of the road who might run across at any instant) over regions of lower criticality (such as buildings in the background, fire hydrants, trees, etc). No such prioritization is done in current machine learning software. Rather, some of the heaviest computational operations are performed on all bits of an image in every frame without prioritization. A novel stack is needed that is aware of importance of different regions in an image. Some examples were proposed in recent literature.  


\subsection{Gaps in the existing solutions}




==> sec_foundations.tex <==
\section{Challenge of Foundations}
As foundation of the IoT system, challenges comes from three aspects -- analytical foundations, architectural foundations, and systems foundations.

\subsection{Analytical Foundations}
We present the analytical foundations necessary for developing IoT systems. Problems include,
\begin{enumerate}
    \item Information theoretic methods to understand the limits of sensing and communication in the systems.
    \item Information theoretic methods to understand the limits of AI especially under resource-constraints for IoT.
\end{enumerate}

\subsection{Architectural Foundations}
Since protocols and each system modules are often designed independently, we need redesign the architectural smartly to combine these protocol and modules together and thus the architectural foundations is the general platform for all kinds of protocols and modules in IoT.

\subsection{Foundations of Systems}
We present the foundations of systems necessary for developing IoT systems. Problems include,
\begin{enumerate}
    \item Actuation in IoT systems requires control under varying delay and unpredictable delivery.
    \item IoT systems need security solutions for the range of heterogeneity and resource constraints seen in IOT settings.
    \item IoT systems need the ability to reason about end-to-end systems properties when humans are in the loop and to provide incentives for their participation.
\end{enumerate}

==> sec_prior_work.tex <==
\section{Prior Works}
% Summarize the prior works in prior_papers.txt

==> structure.tex <==
\begin{enumerate}
\item Introduction \\ {\color{red} 1.5 pages}

\item Systems and networking challenges \\
   {\color{red} 2 pages}
   \begin{itemize}
   \item Unique problems
   \item Requirements
   \item Open Research Problems: For each mention alongside current work and high-level gaps
   \item High-level statement (a few sentences) about research agenda on the topic
   \end{itemize}
   
\item Reliability and security challenges \\
   {\color{red} 2 pages}
   {\color{red} 2 pages}
   \begin{itemize}
   \item Unique problems
   \item Requirements
   \item Open Research Problems: For each mention alongside current work and high-level gaps
   \item High-level statement (a few sentences) about research agenda on the topic
   \end{itemize}
   
\saurabh{The testbed section is optional depending on how much space we have.}
\item IoT testbeds \\
   {\color{red} 1 page}
   \begin{itemize}
   \item Desired characteristics
   \item Current state
   \item Desired end goal
   \end{itemize}
   
\item Key open technical challenges in systems + networking for IoT \\
{\color{red} 0.5 page}
\end{enumerate}

\begin{comment}  
\item Systems and networking challenges \\
   {\color{red} 2 pages}
   \begin{itemize}
   \item Unique problems
   \item Existing foundations we can build on in the areas of: (i) Analytical (ii) Architectural (iii) Systems
   \item Gaps in the existing solutions
   \end{itemize}
   
\item Reliability and security challenges \\
   {\color{red} 2 pages}
   \begin{itemize}
   \item Unique problems
   \item Existing foundations we can build on in the areas of: (i) Analytical (ii) Architectural (iii) Systems
   \item Gaps in the existing solutions
   \end{itemize}
\end{comment}

\begin{comment}   
\item Challenges in applying ML to IoT
\saurabh{Is this going to make the article too diffuse?}

   \begin{itemize}
   \item Unique problems 
   \item Existing foundations we can build on in the areas of: (i) Analytical (ii) Architectural (iii) Systems
   \item Gaps in the existing solutions 
   \end{itemize}
\end{comment}

